Image color consistency in datasets: the Smooth-TPS3D method

Image color consistency is the key problem in digital imaging consistency when creating datasets. Here, we propose an improved 3D Thin-Plate Splines (TPS3D) color correction method to be used, in conjunction with color charts (i.e. Macbeth ColorChecker) or other machine-readable patterns, to achieve image consistency by post-processing. Also, we benchmark our method against its former implementation and the alternative methods reported to date with an augmented dataset based on the Gehler's ColorChecker dataset. Benchmark includes how corrected images resemble the ground-truth images and how fast these implementations are. Results demonstrate that the TPS3D is the best candidate to achieve image consistency. Furthermore, our Smooth-TPS3D method shows equivalent results compared to the original method and reduced the 11-15% of ill-conditioned scenarios which the previous method failed to less than 1%. Moreover, we demonstrate that the Smooth-TPS method is 20% faster than the original method. Finally, we discuss how different methods offer different compromises between quality, correction accuracy and computational load.

==> 3_experiments_table.tex <==
\begin{table}[]
    \centering
    \caption{All the color corrections performed in this work. The table shows the name of the correction, the acronym used in this work to refer to the correction and the augmented definition for each vector of $ P $, the color references or color to be corrected. In this table we use a reduced notation $ \Delta_i =  \Delta_{RGB} (\mathbf{s}_i, \mathbf{c}) $ for simplicity.}
    % \setlength{\tabcolsep}{2em}
    \renewcommand{\arraystretch}{1.6}
    % \begin{footnotesize}
    \scalebox{0.9}{
\begin{tabular}{lrr}
\hline 
\textbf{Correction} & \textbf{Acronym} & \textbf{Color mapping contributions}      \\
\hline 
Perfect   & PERF    & $  (r, g, b) $         \\
No correction  & NONE    & $  (r, g, b) $         \\
\hline
White-balance  & AFF0    & $  (r, g, b) $         \\
White-balance w/ black subtraction & AFF1    & $  (1, r, g, b) $      \\
Affine    & AFF2    & $  (r, g, b) $         \\
Affine w/ translation    & AFF3    & $  (1, r, g, b) $      \\
\hline
Vandermonde (degree=2)    & VAN0    & $  (1, r, g, b, r ^2, g ^2, b ^2) $     \\
Vandermonde (degree=3)   & VAN1    & $  (1, r, g, b, r ^2, g ^2, b ^2, r ^3, g ^3, b ^3 ) $        \\
Vandermonde (degree=3)   & VAN2    & $  (1, r, g, b, r ^2, g ^2, b ^2, r ^3, g ^3, b ^3, r ^4, g ^4, b ^4 ) $       \\
Vandermonde (degree=4)   & VAN3    & $  (1, r, g, b, r ^2, g ^2, b ^2, r ^3, g ^3, b ^3, r ^4, g ^4, b ^4, r ^5, g ^5, b ^5) $  \\
\hline
Cheung (terms=5)     & CHE0    & $  (1, r, g, b, rgb) $      \\
Cheung (terms=7)    & CHE1    & $  (1, r, g, b, rg, rb, gb) $         \\
Cheung (terms=8)    & CHE2    & $  (1, r, g, b, rg, rb, gb, rgb) $         \\
Cheung (terms=10)   & CHE3    & $  (1, r, g, b, rg, rb, gb, r ^2, g ^2, b ^2) $        \\
\hline
Finlayson (degree=2)     & FIN0    & $  (r, g, b, r ^2, g ^2, b ^2, rg, rb, gb) $      \\
Finlayson (degree=3)     & FIN1    &  
$
     (r, g, b, r ^2, g ^2, b ^2, rg, rb, gb, r ^3, g ^3, b ^3,  rg ^2, gb ^2, rb ^2, gr ^2, bg ^2, br ^2, rgb)  
$      \\
Finlayson root (degree=2)     & FIN2    & $  (r, g, b,  \sqrt{rg}, \sqrt{rb},  \sqrt{gb}) $      \\
Finlayson root (degree=3)     & FIN3    & 
$  
(r, g, b,  \sqrt{rg}, \sqrt{rb},  \sqrt{gb},  \sqrt[3]{rg ^2},  \sqrt[3]{gb ^2},  \sqrt[3]{rb ^2}, \sqrt[3]{gr ^2},  \sqrt[3]{bg ^2},  \sqrt[3]{br ^2},  \sqrt[3]{rgb}) 
$ \\
\hline
Thin-plate splines (Manesatti)     & TPS0    & $ (1, r, g, b,  \Delta_1 ^2  \ln  \Delta_1,  \dots,  \Delta_{24} ^2  \ln  \Delta_{24}) $       \\
Thin-plate splines (ours, smooth=0)     & TPS1    & $ (1, r, g, b,  \Delta_1,  \dots,  \Delta_{24}) $        \\
Thin-plate splines (ours, smooth=0.001) & TPS2    & $ (1, r, g, b,  \Delta_1,  \dots,  \Delta_{24}) $        \\
Thin-plate splines (ours, smooth=0.1)   & TPS3    & $ (1, r, g, b,  \Delta_1,  \dots,  \Delta_{24}) $  \\
\hline
\\
\end{tabular}
    }
    % \end{footnotesize}

    \label{tab:correctionssummary}
\end{table}

